Iterative Translation Refinement with Large Language Models

We propose iteratively prompting a large language model to self-correct a translation, with inspiration from their strong language understanding and translation capability as well as a human-like translation approach. Interestingly, multi-turn querying reduces the output's string-based metric scores, but neural metrics suggest comparable or improved quality. Human evaluations indicate better fluency and naturalness compared to initial translations and even human references, all while maintaining quality. Ablation studies underscore the importance of anchoring the refinement to the source and a reasonable seed translation for quality considerations. We also discuss the challenges in evaluation and relation to human performance and translationese.

==> tables/table_automatic_results_gpt_main.tex <==
\small
\setlength{\tabcolsep}{0.58ex}
\begin{tabular}{lcccccccccccccc}
\toprule
& \multicolumn{2}{c}{\scriptsize{WMT21} \small de$\rightarrow$en} 
& \multicolumn{2}{c}{\scriptsize{WMT21} \small en$\rightarrow$de} 
& \multicolumn{2}{c}{\scriptsize{WMT21} \small zh$\rightarrow$en} 
& \multicolumn{2}{c}{\scriptsize{WMT21} \small en$\rightarrow$zh} 
& \multicolumn{2}{c}{\scriptsize{WMT22} \small de$\rightarrow$fr} 
& \multicolumn{2}{c}{\scriptsize{WMT22} \small en$\rightarrow$ja} 
& \multicolumn{2}{c}{\scriptsize{WMT22} \small uk$\rightarrow$cs} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}
& \scriptsize{BLEU} & \tiny{COMET\textsubscript{QE}} & \scriptsize{BLEU} & \tiny{COMET\textsubscript{QE}} & \scriptsize{BLEU} & \tiny{COMET\textsubscript{QE}} & \scriptsize{BLEU} & \tiny{COMET\textsubscript{QE}} & \scriptsize{BLEU} & \tiny{COMET\textsubscript{QE}} & \scriptsize{BLEU} & \tiny{COMET\textsubscript{QE}} & \scriptsize{BLEU} & \tiny{COMET\textsubscript{QE}} \\
\midrule
Reference\textsubscript{A} & - & \textit{.0919} & - & \textit{.1127} & - & \textit{.0708} & - & \textit{\textbf{.0956}} & - & \textit{.0772} & - & \textit{\textbf{.1345}} & - & \textit{\textbf{.1273}} \\
\cdashlinelr{1-15}
Translate & \textbf{30.90} & .1128 & \textbf{25.39} & .1083 & \textbf{25.64} & .0867 & \textbf{29.28} & .0761 & \textbf{36.25}& .0807 & \textbf{23.00} & .1255 & \textbf{29.91} & .1173 \\
Refine & 23.14 & .1116 & 22.35 & \textbf{.1153} & 20.26 & .0921 & 28.26 & .0870 & 32.47 & \textbf{.0851} & 22.63 & \textbf{.1305} & 28.60 & \textbf{.1183} \\
Refine\textsubscript{Contrast} & 22.88 & \textbf{.1162} & 22.54 & .0929 & 24.81 & \textbf{.1132} & \textbf{29.28} & \textbf{.0881} & 33.12 & .0805 & 22.82 & .1282 & 28.90 & .1151 \\
Refine\textsubscript{Random} & 18.83 & .0770 & 19.36 & .0832 & 24.24 & .1022 & 25.71 & .0763 & - & - & - & - & - & - \\
Paraphrase & 11.01 & .0919 & 13.60 & .1006 & 12.76 & .0885 & 21.95 & .0716 & 16.06 & .0682 & 17.69 & .1086 & 13.59 & .0969 \\
\bottomrule
\end{tabular}

